Polynomial invariants by linear algebra

We present in this paper a new technique for generating polynomial invariants, divided in two independent parts : a procedure that reduces polynomial assignments composed loops analysis to linear loops under certain hypotheses and a procedure for generating inductive invariants for linear loops. Both of these techniques have a polynomial complexity for a bounded number of variables and we guarantee the completeness of the technique for a bounded degree which we successfully implemented for C programs verification.

==> invar_eigen.tex <==
\begin{Thm}\labelprop{invar_eigen}
$\varphi : \mathbb{K}^n \mapsto \mathbb{K}$ is a 
semi-invariant if and only if
$\exists \lambda\in\mathbb{K}, \exists \varphi \in E_\lambda, $ where $E_\lambda = ker (f^* - \lambda Id)$.
\end{Thm}


==> invar_eigen_proof.tex <==

\begin{proof}
This comes from a well known linear algebra result : 
\begin{Lemma}\label{dual_stab}
  Let $\mathbb{K}$ be a field, $E$ be a $\mathbb{K}$*vectorial space, 
  $F$ a  sub-$\mathbb{K}$ vectorial space of $E$ and $f : E \rightarrow E$ a linear 
  application.\\
  $f(F) \subset F \Leftrightarrow f^*(F^\bot) \subset F^\bot$
\end{Lemma}
%   We say then that $F$ is stable by $f$. For convenience, we will use the standard 
%   notation $<.,.>$ ($f(x) = <f,x>$).
\begin{proof}
  By linear algebra, we have $<f(x),x'> =<x,f^*(x')>$.
%   
  Let $x\in F, x' \in F^\bot$. 
%   
  If $f(F) \subset F$, then $<f(x),x'> = 0$, so $<x,f^*(x')> = 0$.
%   
  
   As we have $f^*(F^\bot) \subset F^\bot$, we conclude by seeing $(F^\bot)^\bot = F$ 
   and $(f^*)^* = f$. 
$\square$
\end{proof}

Let $Vect(X)$ the vectorial space generated by $X$. 
% 
Let $\varphi$ a semi-invariant, so $(\varphi.x = 0 \Rightarrow \varphi(f(x)) = 0)$.
% 
This means that $Vect(\varphi)^\bot$ is stable by $f$, so by property~\ref{dual_stab}, 
$(Vect(\varphi)^\bot)^\bot = Vect(\varphi)$ is stable by $f^*$. As 
$\varphi \in Vect(\varphi)$, we have $f^*(\varphi) = k*\varphi$.

$\square$
\end{proof}


==> invar_inter.tex <==
\begin{Prop}
 Let $F = \{A_i\}_{1 \leqslant i \leqslant n}$ a family of matrices.
 \begin{equation*}
  Inv(F) = \bigcap\limits_{i=1}^nInv(A_i)  
 \end{equation*}
 
\end{Prop}
 


==> invar_inter_proof.tex <==
\begin{proof}
~

 \begin{Lemma}~\label{inter_lemma}
  
  Let $F=\{A_i\}_{1 \leqslant i \leqslant m},G=\{B_i\}_{1 \leqslant i \leqslant n}$ 
  two matrix families. Then
  $Inv(F\cup G) = Inv (F) \cap Inv(G)$
 \end{Lemma}
 \begin{proof}

 As we have $((p\Rightarrow q) \wedge (p \Rightarrow r)) \Leftrightarrow (p \Rightarrow (q \wedge r))$,
 
  \begin{eqnarray*}
    Inv (F) \cap Inv(G) & = & \{\varphi | \forall X, 
    \begin{array}{llll}
      &(\varphi.X = 0 &\Rightarrow& \bigwedge\limits_{i=1}^m\varphi.A_i.X = 0)\\
           
     \wedge & (\varphi.X = 0&\Rightarrow& \bigwedge\limits_{i=1}^n\varphi.B_i.X = 0)\\
    \end{array}
    \}\\
    ~ & = & \{\varphi | \forall X, \varphi.X = 0 \Rightarrow (\bigwedge\limits_{i=1}^m\varphi.A_i.X = 0 \wedge \bigwedge\limits_{i=1}^n\varphi.B_i.X = 0)\}\\
     ~ & = & Inv(F\cap G)
  \end{eqnarray*}
  
  $\square$

 
 \end{proof}

 By recurrence over the size $n$ of a family $F$, if $n$ equals 1 it is 
 true. If it is true for a certain $n$, then 
 $Inv(F \cup \{A\}) = Inv (F) \cap Inv(\{A\})$ by the previous lemma.
 
 $\square$
% 
%  Let $\varphi$ a element of $\mathbb{K}^n$, and $F = \{A_i\}_{1 \leqslant i \leqslant n}$. 
%  If $\varphi \in Inv(F)$, then it means that
% \\
% By reccurence over the size of the family, we want to show that 
% $\varphi \in \bigcap\limits_{i=1}^nInv(A_i) \Rightarrow \varphi \in Inv(F)$.
% For $n = 1$, the result is implied by the property~\ref{invar_eigen}.
% For $n = 2$, 
% If it is true for a certain $n$, then 


\end{proof}


==> linearizable.tex <==
 \begin{Prop}\labelprop{linear}
  For every solvable polynomial mapping $g$, $g$ is linearizable.
 \end{Prop}
 

==> linearizable_proof.tex <==
  \begin{proof}
 Let $g \in\mathbb{Q}[x]^m$ be a solvable polynomial mapping. There exists a partition of variables
  $x = w_1\cup ...\cup w_k$ such that
  
 \begin{equation*}
  g_{w_j}(x) = M_jw_j^T + P_j(w_1,...,w_{j-1})
 \end{equation*}
 
 We proceed by induction on the size $k$ of the partition on the variables of $g$. We can state that : 
 \begin{itemize}
  \item [$\bullet$] If $k=1,~x = w_1$, then $g_{w_1}(x) = M_1w_1^T + P_1$,
  where $P_1$ is a constant. Then it is clear that $g_{w_1}$ is an affine transformation.
  
  \item [$\bullet$] Assume we can compute a linear application $f$ 
  from $g$ such that $(g(x),P(g(x))) = f(x,P(x))$ if there exists a partition 
  of $k$ sets of variable satisfying the solvable hypothesis. 
%   
  Let $h$ be a solvable polynomial mapping for which there 
  exists a partition of $x$ into $k+1$ subvectors of variables $x = w_1\uplus ...\uplus w_{k+1}, 
  w_i\cap w_j = \emptyset$ if $i \neq j$.
%  
  By induction hypothesis, we can linearize $h_{w_{i}}$ for $1\leqslant i \leqslant k$. 
%   
  Now, the key point is to find a way to linearize 
  \begin{equation*}
  h_{w_{k+1}}(x) = M_{k+1}w_{k+1}^T + P_{k+1}(w_1,...,w_k)
 \end{equation*}
%  
 First, let's note that no variable of $w_{k+1}$ have been used in any other 
 $h_i$. 
%  
 Let $v =\prod\limits_{i=0}^n v_i^{\lambda_i}$ a product of variables in $(w_1\cup...\cup w_k)$. 
 It can appear in $P$ as $v^d$, where $d$ in an integer. We know, by induction hypothesis, that the 
 evolution of $v_i$ following the $h$ transformation can be expressed as a linear application $f$
 with the help of extra variables.
%  Then, let $v_2,...v_{d-1}$ new variables such that
%  $v_i' = (f(v,\mu(x)))^i$.

%   \begin{Lemma}
%    Let $f : \mathbb{K}^n\mapsto \mathbb{K}^2$ a linear application. 
%    There exists a linear application $g:\mathbb{K}^3\mapsto \mathbb{K}^3$ such that 
%    for all $n \in\mathbb{N}$, $(x',y') = f^n(x,y) \Rightarrow (x',y',xy',x_2', y_2') = g^n(x,y,x*y,x^2,y^2)$,
%    with $xy' = x' * y', x_2 ' = x'^2, y_2 ' = {y'} ^2$.
%    
%   \end{Lemma}
  \begin{Lemma}~\label{lem:lin}
   Let $g : \mathbb{K}^n\mapsto \mathbb{K}^n$ a linear application. 
   There exists a linear application $f:\mathbb{K}^m\mapsto \mathbb{K}^m$ with 
   $m \geqslant n$ such that for all $k\in\mathbb{N}$ and $P \in (\mathbb{K}[X])^{m-n}$, $X' = g^k(X) \Rightarrow (X',P(X')) = f^k(X,P(X))$
   
  \end{Lemma}
  
  \begin{proof}
  
  First, let's prove it for $n = 2$ and $P(x,y) = (x.y,x^2, y^2)$.
  Let $g(x,y) = (ax + b_xy, a_yx + b_yy)$.
  Then, $(x.y)' = a_x.a_yx^2 + (a_x.b_y + a_y.b_x)x.y+ b_x.b_y.y^2$, 
  which is a linear combination of $x^2, y^2$ and $xy$.
  Similarly, $(x^2)'$ and $(y^2)'$ can be expressed as linear combinations
  of $x^2$, $y^2$ and $x.y$.
  
  Next, if the degree of the polynomial is $1$, one just need to take $f = g$.
  To generalize this proof for all degrees polynomials, let's assume 
  that for $d \in N$, the lemma is true with $P$ of degree $d$. 
  To express a polynomial of degree $d+1$, one need to express all monomials $m_{d+1}$
  of degree $d+1$, which is the product of a variable $x$ and a monomial $m_d$ of 
  degree $d$. By hypothesis, the monomial of degree $d$ is expressible in $g$ 
  as a linear combination of lower or equal degree monomials. Considering $m_d$ 
  as a variable of $g$, the variable for which we seek a linear representation
  is the product of the two variables $x$ and $m_d$, a case which has been 
  treated before.
  $\square$
  \end{proof}
  
%   This lemma is generalizable for more variable by treating variables by pairs, which
%   leads to the conclusion that the variable $v$ can be expressed by a linear combination
%   of variables, themselves elvolving linearly, so does $v^d$ and any product of powers
%   of variables for the same reason. 
  We can then use Lemma~\ref{lem:lin} to linearize all monomials of elements of
  $w_1, ..., w_k$ occuring in $P$. In the end, we can write h as a linear 
  application over the initial variables and the auxiliary variables introduced
  by the linearization.
  $\square$
 \end{itemize}
 
 \end{proof}

==> movable_constants.tex <==
 \begin{Prop}\labelprop{mov_const}
 Let $\mathcal{F}$ a semi-invariant expressed as 
$\mathcal{F} = \sum\limits_{i=0}^nk_ie_i$.

If $\scalprod{e_0}{X_{init}} \neq 0$, then we have that
\begin{equation*}
\bigwedge\limits_{i = 1}^n (\scalprod{e_i}{X} = -\frac{\scalprod{e_i}{X_{init}}}{\scalprod{e_0}{X_{init}}}\scalprod{e_0}{X})\mathrm{~is~an~invariant} \Leftrightarrow \scalprod{\mathcal{F}}{X_{init}} = 0
\end{equation*}

% are all semi-invariants.
% $k$ such 
%  that $\mathcal{F}' = k.e_j + \sum\limits_{i=0,i\neq j}^ne_i$ with 
%  ($\mathcal{F}$ semi-invariant and $\scalprod{\mathcal{F}}{X} = 0$ satisfiable)
%  $\Rightarrow (\mathcal{F}'$semi-invariant and $\scalprod{\mathcal{F}'}{X} = 0$
%  satisfiable)
 \end{Prop}
 

==> movable_constants_proof.tex <==
 \begin{proof}
 
~

$
  \begin{array}{lcl}
   \scalprod{\mathcal{F}}{X_{init}} = 0 & \Leftrightarrow & \scalprod{\sum\limits_{i=1}^nk_ie_i}{X_{init}} = -k_0\scalprod{e_0}{X_{init}}\\
   ~ & \Leftrightarrow & \sum\limits_{i=1}^nk_i\scalprod{e_i}{X_{init}} = -k_0\scalprod{e_0}{X_{init}}\\
   ~ & \Leftrightarrow & \frac{\sum\limits_{i=1}^nk_i\scalprod{e_i}{X_{init}}}{\scalprod{e_0}{X_{init}}} = -k_0
  \end{array}
$


Let $g(c_1,...,c_n) = -\frac{\sum\limits_{i=1}^nc_i.\scalprod{e_i}{X_{init}}}{\scalprod{e_0}{X_{init}}}$.
% 
We have $g(u_i) = -\frac{\scalprod{e_i}{X_{init}}}{\scalprod{e_0}{X_{init}}}$
% 
We note that $g$ is linear, thus :

$
  \begin{array}{lcl}
   \scalprod{\mathcal{F}}{X_{init}} = 0 & \Leftrightarrow & g(k_1,...,k_n)\scalprod{e_0}{X_{init}} = \sum\limits_{i=1}^nk_i\scalprod{e_i}{X_{init}}\\
   ~ &\Rightarrow& \bigwedge\limits_{i = 1}^n (\scalprod{e_i}{X} = -\frac{\scalprod{e_i}{X_{init}}}{\scalprod{e_0}{X_{init}}}\scalprod{e_0}{X})\\
  \end{array}
$

by setting $k_i = 1$ and $k_j = 0$ for all $j \neq i$.

Now to prove that this transformation does not make us lose precision, we will construct $\mathcal{F}$ with the $n$ equations.

  If $\bigwedge\limits_{i = 1}^n (\scalprod{e_i}{X} = g(u_i)\scalprod{e_0}{X})$, then as $g$ is a linear application
  we have that 
  \begin{equation*}
   \sum\limits_{i=1}^n k_i\scalprod{e_i}{X} = g(k_1,...,k_n)\scalprod{e_0}{X}
  \end{equation*}

  We conclude by setting $k_0$ to $-g(k_1,...,k_n)$

  $\square$
 \end{proof}
 


==> num_variables.tex <==
\begin{Prop}\labelprop{num_var}

Every solvable polynomial mapping $g$ using $n$ variables is linearizable 
by a linear mapping $f$ using at most
${n+d \choose d}$ new variables, where $d$ is the degree of $P$, the
polynomial linearizing $g$ as in definition~\ref{def:linearizable}.

\end{Prop}


==> num_variables_proof.tex <==
 

\begin{proof}

This property comes from~\cite{muller2004precise}. ${n+d \choose d}$
is the total number of variables needed to express all monomials products
of $n$ variables of degree lower or equal to $d$. 
%  Let $d$ the polynomial degree and $(x_1,x_2,...,x_n)$ the variables.
% %  
%  In the worst case, we will need as much variables as combinations of variables
%  products.
% %  
%   We search for the number of power repartition $(i_1,i_2,...,i_n)$ over 
%   variables such that $\Sigma_{j=1}^n i_j \leqslant d$. Let's note this 
%   value $C(d,n)$.
% % 
%  \begin{Lemma}\label{multi_newt}
%   $\forall d, n \in\mathbb{N}, |\{(i_1,...,i_n). \forall j, i_j \geqslant 0, \Sigma_{j=1}^n i_j = d\}| = {n+d-1 \choose d}$
%  \end{Lemma}
%  \begin{proof}
%  
%   Newton's multinom.
%  $\square$
%  \end{proof}
%  
%  We have :
%  
%  \begin{eqnarray*}
%   C(d,n) &=&  {n+d \choose d} \\
%   \xspace &=& \{(i_1,...,i_n). \forall j, i_j \geqslant 0, \sum_{j=1}^n i_j \leqslant d\}|\\
%   \xspace &=& \sum_{i=1}^{d}(|\{(i_1,...,i_n). \forall j, i_j \geqslant 0, \sum_{j=1}^n i_j = i\}|)\\
%   \xspace &=& \sum_{i=1}^{d} {n+i-1 \choose i}~\mathrm{by~Lemma~\ref{multi_newt}}\\
%  \end{eqnarray*}
%  
%  By recurrence over $d$, we have 
%  
%  \begin{eqnarray*}
%   C(d+1,n) &=&\{(i_1,...,i_n). \forall j, i_j \geqslant 0, \sum_{j=1}^n i_j \leqslant d+1\}\\
%   \xspace &=& \sum_{i=1}^{d+1}(|\{(i_1,...,i_n). \forall j, i_j \geqslant 0, \sum_{j=1}^n i_j = i\}|)\\
%   \xspace &=& \sum_{i=1}^{d+1} {n+i-1 \choose i}\\
%   \xspace &=& {n+d \choose d+1} + \sum_{i=1}^{d} {n+i-1 \choose i}\\
%   \xspace &=& {n+d \choose d+1} + {n+d \choose d} \mathrm{par~hypothese~de~recurrence}\\
%   \xspace &=& {n+d+1 \choose d+1} 
%  \end{eqnarray*}
%  $\square$
\end{proof} 


==> prod_eigen.tex <==
 

  \begin{Prop}\labelprop{shape_ev_monoms}
  Let $A\in\mathcal{M}_d(\mathbb{Q}),\Lambda(M)$ the eigenvalue set of a
  matrix $M$ and $d$ an integer.
%   
  Then for any product $p$ of $d$ or less elements of $\Lambda(A), p \in \Lambda(\Psi_d(A))$.
  
  
%   Let $A\in\mathcal{M}_n(\mathbb{Q}),\lambda,\lambda'$ two complex eigenvalues
%   of $A$. Let $J$ be the normal Jordan form of $A$ and $x,y$ variables respectively associated to $\lambda$ and $\lambda'$. 
%   The presence of a variable representing $x.y$ induces the presence of the 
%   eigenvalue $\lambda.\lambda'$.
  
  \end{Prop}


==> prod_eigen_proof.tex <==
  \begin{proof}
  
  First of all, we will prove some simple properties about $\Psi_d$.
  
  \begin{Lemma}~\label{psi_assoc}
    \begin{enumerate}
      \item  $\Psi_k(A.B) = \Psi_k(A).\Psi_k(B)$ 
      \item  $\Psi_k(A^{-1}) = \Psi_k(A)^{-1}$ 
      
    \end{enumerate}
  \end{Lemma}
  \begin{proof}    
    \begin{enumerate}
      \item $\Psi_k(A).\Psi_k(B)p(X)= \Psi_k(A).p(B.X) = p(A.B.X) = \Psi_k(A.B)p(X)$
      \item $\Psi_k(A^{-1}).\Psi_k(A) . p(X) = p(A.A^{-1}X) = p(X)$
      so $\Psi_k(A^{-1}).\Psi_k(A) = Id$.
    \end{enumerate}
  $\square$
  \end{proof}
  
  To deal with this, let's consider $J$ the Jordan normal form of $A$. 
  As we are working with $\mathbb{C}$, which is an algebraically closed field,
  $A$ is similar to $J$ (ie. $\exists P. A = P^{-1}JP$), with 
  
      $J =\left(
	  \begin{array}{cccc}
	    J_1 & 0 &... &0\\
	    0 & \ddots &  \ddots & \vdots\\
	    \vdots & \ddots & \ddots & 0\\
	    0 & ... & 0 & J_k
	    \end{array}\right) $,
% 	    
	    and
% 	    
	    $J_k = \left(
	  \begin{array}{cccc}
	    \lambda_k & 1 &  ... &0\\
	    0 & \ddots  & \ddots &\vdots\\
	    \vdots & \ddots & \ddots & 1\\
	    0 & ... & 0 & \lambda_k
	    \end{array}\right) $
  
  As $A = P^{-1}JP,~\Psi_k(A) = \Psi_k(P)^{-1}.\Psi_k(J)\Psi_k(P)$, so 
  $\Psi_k(A)$ is similar to $\Psi_k(J)$.
%   
  This means that they have the same set of eigenvalues.
% 
  The transformation of a variable $x$ by $J$ can be either of the form 
  $\lambda.x$, either $\lambda.x + y$, with $\lambda$ an eigenvalue of $J$
  and $y$ another variable.
% 
  Another interesting information from the jordan normal form is that this 
  variable $y$ does not depend on $x$.
% 
To understand the proof, let's see what happens for $d = 2$ and $n = 2$.

If $\lambda$ and $\lambda'$ are
   eigenvalues of $A$, then $J =\left(
  \begin{array}{cc}
    \lambda & b\\
    0 & \lambda'
  \end{array}\right)$ with $b = 0$ or $1$ .
%   
  So $\Psi_2(J) = \left(\begin{array}{ccccc}
    \lambda^2  & 2\lambda\lambda'& \lambda'^2 & 0 & 0\\
    0  & \lambda\lambda'& b\lambda' & 0 & 0\\
    0 & 0 & \lambda'^2 & 0 & 0\\
    0 & 0 & 0 & \lambda & b\\
    0 & 0 & 0 & 0 & \lambda'
  \end{array}\right)$. 
  
  $\Psi_2(J)$ is upper triangular, so its eigenvalues are on the diagonal : 
  $\lambda, \lambda', \lambda^2, \lambda\lambda'$ and $\lambda'^2$
  
The proof for any number of variables and any degree is similar. 
%     
  We just need to analyse the elevation of the Jordan normal form of $A$.
%   
    
  \begin{Def}
   Let $f$ a linear application. We define a 
   \emph{dependency order} $\prec_f$ on $Var$ a total order such that 
   for all $x \in Var$, $f(X)$ restricted to $x$
   depends only on a linear combination of variables $V$ for which 
   $\forall y \in V, y \preceq_f x$. We also say that $f$ respects $\prec_f$.
  \end{Def}
  The idea behind this is that an upper-triangular matrix $J$ induces such an 
  order : 
  the last element $x_n$ only depend on himself, the previous element $x_{n-1}$
  depends on himself and $x_n$, so $x_n \prec_A x_{n-1}$, etc..
  We note that for any triangular matrix, the diagonal coefficients are
  the eigenvalues of the said matrix and of all similar matrix. 
%   
%   The relation between two successive variables induces an order on the variables. 
%   
%   Thus :
%   
%   \begin{Lemma}
%    Let $\mathbb{K}$ a field,  $f : \mathbb{K}^n \rightarrow \mathbb{K}^n$ a 
%    linear application whose matrix is triangular, $x\in Var$ and $\prec_f$ a 
%    dependency order. If there exists a relation of the form 
%    $x' = \lambda.x + l$, with $l$ a linear combination of variables 
%    $y \prec_f x$ with $f$ respecting $\prec_f$
%    then the eigenvalue associated to $x$ is $\lambda$.
%   \end{Lemma}

  In other words, if for the $i^{th}$ variable of an application,
  the line of its matrix is composed of $i-1$ zeros then $\lambda$
  at the $i^{th}$ position, then its eigenvalue is $\lambda$.

We define $\prec_J$ as an order that $J$ respects.
% 
By choosing a right order for monomials of $p$, we will show that $\Psi_k(J)$ 
is upper-triangular.
% 
We will take the graded lexicographic order $\prec^g_J$ with respect to $\prec_J$, i.e. 
the order such that : 
\begin{itemize}

  \item if $x \prec_J y$ two variables, then $x \prec^g_J y$ ;
  \item if $m_1 \prec^g_J m_2$, then for any monomial $m_3$, 
  $m_1.m_3 \prec^g_J m_2.m_3$.

\end{itemize}

If $x \prec_J^g y$ then by definition $x \prec_J y$.
% 
Moreover, $m_1 \prec^g_J m_2 \Leftrightarrow (m_1$ does not appear in the 
expression of $m_2)$, then let $m_3$ any monomial.
% 
We can clearly see that $m_1.m_3$ does not appear in the expression of 
$m_2.m_3$. Thus : 
\begin{Lemma}\label{glo_dep_order}
 Let $J$ an upper triangular matrix, $\prec_J$ be a dependency order
 respected bu $J$.
 Then for any $k \in \mathbb{N}$, $\prec^g_J$ can be a dependency order for 
 $\Psi_k(J)$.
\end{Lemma}
  
  By our construction of the linearization process of~\ref{poly2lin}, we can 
  state that for all $x,y,z \in Var$, if $x \prec_J y \preceq_J z$,
  then $y^iz^j \prec^g_J x^{i+j}$ is impossible for all $i,j$
  as $x$ does not depend on $y$ or $z$, but the contrary is false. Thus :
  
  \begin{Lemma}~\label{order_stable}
   Let $f$ a linear application, $\prec_f$ a dependency order on $f$, 
   $x,y \in Var$. Let $Mon_d(x,y)$ the set of variables representing 
   monomials of degree lower or equal to $d$ depending on $x$ and $y$. Then 
   $z \prec_f x \prec_f y \Rightarrow v \in Mon_d(x,y), z^d \preceq_f^g v$.
%    and
%    $\forall d'<d, \forall v' \in Mon_{d'}(x,y), v' \prec v $
  \end{Lemma}

  In other words, in a triangular matrix $M$ representing $x,y,z$ and its monomials,
  if $x$ and $y$ are over $z$ and $M$ respects $\prec_M^g$, then $x^i.y^j$ will always be over $z^k$, for 
  every $i,j,k$ with $k \leqslant i + j$.

  Let $x,y,z,t$ 
  variables such that $x' = \lambda_x.x + j_zz$, and $y' = \lambda_y.y + j_tt$  
  where $j_z$ and $j_t = 0$ or $1$. Then the matrix $\Psi_k(J)$ will set 
  $x^i.y^j$ to $(\lambda_x.x + j_zz)^i(\lambda_y.y + j_tt)^j$. 

Eventually, when one develop $x^i.y^j$, there is : 
\begin{enumerate}
 \item[$\bullet$] $0$ for  \emph{monomial variables} of strictly higher 
 degree ;
 \item [$\bullet$] $0$ for \emph{monomial variables} containing $t$ such
 that $t \prec x \prec y$ by lemma~\ref{order_stable} ;
 \item [$\bullet$] $0$ for monomials $x^{i'}.y^{j'}$ with $i' + j' = d$ 
 and $i' > i$ ; 
 \item [$\bullet$] a coefficient $\lambda_x^i.\lambda_y^j$ for the variable 
 $x^i.y^j$, which will be on the diagonal of $\Psi_k(J)$.
\end{enumerate}

The third point is true because if $x \prec_J y$, then 
$x^iy^{j} \prec_J^g x^{i-1}y^{j+1}$ and $\prec_J^g$ is a dependency order
for $\Psi_k(J)$~\ref{glo_dep_order}.

$\Psi_k(J)$ will be upper-triangular itself by respecting $\prec^g_J$.
% \vspace{1ex}
% To treat additions is easier. Let $x,y$ two variables. Then, to represent 
% $x+y$, we just need to see that 
% $(x+y)'=(\lambda_x + \lambda_y)(x + y)+(a+c-\lambda_x)x + (b + d - \lambda_y)y$

$\square$

  \end{proof}
